TeleFMG: A Wearable Force-Myography Device for Natural Teleoperation of Multi-finger Robotic Hands

Teleoperation enables a user to perform dangerous tasks (e.g., work in disaster zones or in chemical plants) from a remote location. Nevertheless, common approaches often provide cumbersome and unnatural usage. In this letter, we propose TeleFMG, an approach for teleoperation of a multi-finger robotic hand through natural motions of the user's hand. By using a low-cost wearable Force-Myography (FMG) device, musculoskeletal activities on the user's forearm are mapped to hand poses which, in turn, are mimicked by a robotic hand. The mapping is performed by a spatio-temporal data-based model based on the Temporal Convolutional Network. The model considers spatial positions of the sensors on the forearm along with temporal dependencies of the FMG signals. A set of experiments show the ability of a teleoperator to control a multi-finger hand through intuitive and natural finger motion. A robot is shown to successfully mimic the user's hand in object grasping and gestures. Furthermore, transfer to a new user is evaluated while showing that fine-tuning with a limited amount of new data significantly improves accuracy.

==> design.tex <==
FMG wearable device -
In a previous paper we have developed a prototype of a low-cost wearable device for identifying objects in a user's hand which imply about the intended task, uses Force-Myography (FMG) [Nadav quote]. In this paper we have developed  a second generation of this device, which is mostly 3D printed, uses Force-Myography (FMG) to capture musculoskeletal activities via force sensors on the human arm. The FMG device is simple, low-cost and quite comfortable. 
The device is composed of 28 low-cost FSR sensors, specifically the FSR 400 short-tail model by Interlink Electronics. FSR sensors are composed of thin sheets of polymer that alter their electrical resistance in response to the amount of pressure applied to their surface.
The device that can be seen in Figure (1), consists of three main components: (a) upper forearm band with 14 FSR sensors organized in two rows, (b) lower forearm band with 14 sensors organized in two rows and (c) a processing unit, based on Teensy 4.1,microcontroller, which allows for the connection of up to 18 analog channels, and 600 MHz processing speed.
Since the unit has the option of connecting 18 analog channels, the force sensors will be divided into two groups of sensors, two analog sensors from a separate set will be connected to each analog input in the controller through a voltage divider of $4.7k\Omega$ resistor. Using a switching system at any given time the controller will sample a different set of sensors cyclically. The
FSR sensors were positioned in equal spacing along the bands. 
The bands were fabricated by 3D printing with an elastic polymer (Thermoplastic elastomer). They include a button for each sensor that is adjacent to the arm and presses the sensor. The system is flexible and allows unrestricted movement of the entire arm.
The system can receive samples at a practical rate of 40 Hz.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/FMG_wd.png}
    \caption{FMG wearable device.}
    \label{fig:example}
\end{figure}

Sensor glove - 
In addition to the FMG wearable device, we developed a sensor glove in order to measure the position of the hand, the system allows us to measure the angles of the fingers, which will be used as ground true, for the deep learning model later.
The sensor glove that can be seen in Figure (2), consists of two main components: (a) A cloth glove on which there are 10 A fabric glove on which there are 10 sensors, 5 flex sensors (Flex Sensor 2.2" SEN-10264 ROHS by Spectra Symbol), for measuring metacarpophalangeal joints angles, and 5 potentiometers (PT15NH05-103A2020-S by Amphenol Piher), for measuring proximal interphalangeal angles joints. These sensors are connected to the glove using 3D printed  connectors printed.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.25\textwidth]{Figures/sensor_glove.png}
    \caption{Sensor glove.}
    \label{fig:example}
\end{figure}

==> related_work.tex <==
related work -
